Interface Automata for Choreographies

Choreographic approaches to message-passing applications can be regarded as an instance of the model-driven development principles. Choreographies specify interactions among distributed participants coordinating among themselves with message-passing at two levels of abstractions. A global view of the application is specified with a model that abstracts away from asynchrony while a local view of the application specifies the communication pattern of each participant. Noteworthy, the latter view can typically be algorithmically obtained by projection of the global view. A crucial element of this approach is to verify the so-called well-formed conditions on global views so that its projections realise a sound communication protocol. We introduce a novel local model, group interface automata, to represent the local view of choreographies and propose a new method to verify the well-formedness of global choreographies. We rely on a recently proposed semantics of global views formalised in terms of pomsets.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{M. Bartoletti, L. Henrio, A. Mavridou, A. Scalas (Eds.):\\
12th Interaction and Concurrency Experience (ICE 2019).\\
EPTCS 304, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.304.1}{10.4204/EPTCS.304.1}}

